Multi-Spectral Image Synthesis for Crop/Weed Segmentation in Precision Farming

An effective perception system is a fundamental component for farming robots, as it enables them to properly perceive the surrounding environment and to carry out targeted operations. The most recent methods make use of state-of-the-art machine learning techniques to learn a valid model for the target task. However, those techniques need a large amount of labeled data for training. A recent approach to deal with this issue is data augmentation through Generative Adversarial Networks (GANs), where entire synthetic scenes are added to the training data, thus enlarging and diversifying their informative content. In this work, we propose an alternative solution with respect to the common data augmentation methods, applying it to the fundamental problem of crop/weed segmentation in precision farming. Starting from real images, we create semi-artificial samples by replacing the most relevant object classes (i.e., crop and weeds) with their synthesized counterparts. To do that, we employ a conditional GAN (cGAN), where the generative model is trained by conditioning the shape of the generated object. Moreover, in addition to RGB data, we take into account also near-infrared (NIR) information, generating four channel multi-spectral synthetic images. Quantitative experiments, carried out on three publicly available datasets, show that (i) our model is capable of generating realistic multi-spectral images of plants and (ii) the usage of such synthetic images in the training process improves the segmentation performance of state-of-the-art semantic segmentation convolutional networks.

==> guiimage.tex <==
gui


==> olds/abstract.tex <==
An effective perception system is a fundamental component for farming robots, as it enables them to properly perceive the surrounding environment and to carry out targeted operations. The most recent approaches make use of state-of-the-art machine learning techniques to learn an effective model for the target task. However, those methods need a large amount of labelled data for training. A recent approach to deal with this issue is data augmentation through Generative Adversarial Networks (GANs), where entire synthetic scenes are added to the training data, thus enlarging and diversifying their informative content. 

In this work, we propose an alternative solution with respect to the standard data augmentation techniques, applying it to the fundamental problem of crop/weed segmentation in precision farming. Starting from real images, we create semi-artificial samples by replacing the most relevant object classes (i.e., crop and weeds) with synthesized counterparts. To do that, we employ a conditional GAN (cGAN), where the generative model is trained by conditioning the shape of the generated object. Moreover, in addition to RGB data, we take into account also near-infrared information, generating 4 channel multi-spectral synthetic images.
%To achieve this, we propose a conditional GAN (cGAN), where the generative model is trained conditioning the shape of the generated object. Therefore, by providing as input conditions shapes of real objects, the generative model will synthesize new realistic objects while keeping their original footprint onto the image. Finally, the proposed generative architecture will also take into account the near-infrared information, generating 4 channel multi-spectral synthetic images.
%To corroborate the effectiveness of the proposed architecture we report
Quantitative experiments, carried out on two publicly available datasets, show that 1) our model is capable of generating realistic multi-spectral images of plants, and 2)  the usage of such synthetic images in the training process improves the segmentation performance of state-of-the-art semantic segmentation Convolutional Networks.

==> olds/conclusions.tex <==
This paper introduces a data augmentation strategy that leverages a cGAN to generate entire agricultural scenes by synthesizing only the most relevant objects for segmentation purposes. The core of the proposed approach consists of exploiting the shapes of real objects to condition the trained generative models. The existing shapes are extracted from real-world labeled images. In addition, the generation process also synthesizes the NIR channel. The obtained synthetically augmented dataset can then be used to train a semantic segmentation network. We applied this method to the crop/weed segmentation process, a well-known problem in agricultural robotics, showing that the cGAN augmented datasets can improve the performance of different state-of-the-art segmentation architectures.

\balance

==> olds/introduction.tex <==
Precision Agriculture is a farming management concept based on observing, measuring, and responding to inter- and intra-field variability in crops \cite{LEE20102}. A key objective is the minimization of environmental impact by reducing the reliance of chemicals products such as herbicides or pesticides.
Farming robots can play an important role in this mission, since they can carry out a precise weed control by selective treatment applications. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=.7\columnwidth]{images/intro_reduced.png}
    \caption{ Top row: The BOSCH Bonirob farming robot used to collect the datasets considered in the experiments. Bonirob is equipped with a Weed Intervention Module (the black structure between the wheels in the picture). This module consists of a perception system for weed classification and a multi-modal actuation systems for weeds removal. Middle row: From left to right, synthetic RGB and NIR samples, respectively. Bottom row: From left to right, the pixel-wise ground truth and the FCN segmentation result, respectively.}
    \label{fig:teaser_img}
\end{figure}

A fundamental requirement to perform selective treatments through robots is to build an effective perception module capable of identifying and localizing crop and weeds in the field and thus to 
% (e.g., see Fig. \ref{fig:teaser_img}, top).
%The locations of crop and weeds are used to
trigger the proper weeding actions. 
The most commonly adopted approaches use vision-based approaches to tackle this problem, and rely on machine learning methods, such as Convolutional Neural Networks (CNNs)
\mbox{\cite{potena2016,lottesJFR2016,weednet}}. These data-driven methods allow to train powerful visual classifiers that report high classification performance. However, their performance strongly depends on the size and variety of the training dataset~\cite{xie2016}. This problem is well-know and has been addressed in many different ways (among others, \cite{potena2016,dicicco2017}). More recent approaches address this problem by leveraging Generative Adversarial Networks (GANs)~\mbox{\cite{valerio2017arigan,sixt2018rendergan}}. These methods allow to train, in an unsupervised manner, powerful generative models capable to synthesize photo-realistic images that are used to increase and diversify the original training datasets. This results in an improved generalization capability of the learned visual classifiers.\\

In this work, we propose a novel methodology to synthesize photo-realistic images by using a generative adversarial method. Unlike the conventional use of GANs, which aims to train a model to generate an entire scene, we generate semi-artificial images by replacing with synthesized, photo-realistic, counterparts only the scene objects that belong to the object classes that are relevant to the target perception task (e.g., crop, weed plants in our case). 

The main intuition behind this idea is that, usually, vision-based learned classifiers are not able to equally generalize across all the target classes, which in turn can lead to unbalanced classification performance. Given that, the proposed method exploits a GAN to only learn the data distribution associated to a subset of the target classes, allowing to train more compact generative models and to create photo-realistic training samples in a faster and more effective way.

To achieve our goal, we use a conditional GAN (cGAN), where the generative model is trained by conditioning the shape of the generated object. Therefore, by providing as an input constraint the object shapes extracted from real objects, the generative model will synthesize new realistic objects while keeping their original footprint onto the image. Moreover, our generative architecture will also take into account near-infrared information, generating 4 channel multi-spectral synthetic images. %Finally, the generated samples are replaced to their real counterparts.

To evaluate the effectiveness of the proposed architecture, we report experiments on two publicly available farming datasets, showing that our model is capable to generate realistic $512\times512$ multi-spectral images of plants, and that the usage of these synthetic images during the training process improve the segmentation performance of state-of-the-art Fully Convolutional Networks (FCNs).


% The proposed approach is evaluated in a sugarbeet precision farming scenario. We generate synthetic datasets to training different state-of-the-art segmentation networks, showing how the proposed methods for synthetic image generation properly generalizes across different segmentation approaches.

==> olds/methods.tex <==
The main objective of the proposed approach is to develop an algorithm capable of synthesizing realistic agricultural scenes. Let us define our data distribution $p_{data}(x)$ as a set of images collected by a moving robot in a sugar beet field. The images are acquired by a multi-spectral camera that collects Near-Infrared (NIR) images in addition to, and registered with, RGB images. The dataset is annotated in a pixel-wise manner.
%(see Fig. \ref{fig:teaser_img}).

We want to learn a function $G : z , y \rightarrow x$ that maps the input mask $y$ to a realistic multi-spectral image. The mapping function $G$ is implemented in a cGAN that contains an implicit model of the conditional probability distribution $p(x|y)$ learned by training. The resulting images will be used as data augmentation to train a deep learning model for crop/weed segmentation. This pipeline enables to enlarge and to diversify the training dataset, and thus to significantly improve the generalization of deep learning models. 

The usage of cGAN as data augmentation tool is not novel and it has been explored in different fields, ranging from medical images, anomaly detection, image classification, and even to decode the position, orientation, and binary ID of markers \cite{DBLP:journals/corr/abs-1709-00938, DBLP:journals/corr/SixtWL16,8363678}. cGANs have not been extensively adopted in image segmentation contexts yet. In this regard, we propose a method that synthesizes full agricultural scenes.

A similar problem is usually addressed by training a generative model capable to reproduce an entire scene, which requires deep models, a large amount of training data, and a high computational power. However, by considering that the goal is to achieve data augmentation for the training dataset, a full scene generation is redundant. Moreover, since the accuracy of a FCN can often vary  significantly across classes, it is interesting to augment the number of training samples only for the classes with a lower classification accuracy. For example, in a crop/weed segmentation scenario, a network usually tends to accurately detect the terrain, while it usually miss-classifies the pixels belonging to crop and weeds due to their similar visual appearance. In such a scenario, it is redundant to increase the number of terrain samples, while increasing the crop samples can provide a significant information gain.

In this work, rather than training a generator $G$ capable to synthesize an entire scene, our idea is to focus on generating instances of some specific object classes, specifically the ones with the lowest segmentation accuracy. In the rest of this section, we describe the three major steps involved in the generation of realistic agricultural samples:

\begin{enumerate}
% \item[i)] The RGB-NIR image generation process is described in Section \ref{sec:rgb_nir};
%\item[i)]
\item The training of the cGAN for learning the generative model. % $G$ is described in Section \ref{sec:cgan};
%\item[ii)]
\item The quantitative evaluation of cGAN training results. %the metrics employed to evaluate the  are reported in Section \ref{sec:gan_train_ev};
%\item[iii)]
\item The composition of the synthetic farming scenes.% is described in Section \ref{sec:scene_gen}.
\end{enumerate}

% \subsection{RGB-NIR dataset generation}
% \label{sec:rgb_nir}

% The first step of our approach concerns the generation of agricultural scenes populated by synthetic crop samples. A similar problem is usually addressed by training a generative model capable to reproduce an entire scene, which requires deep models, a large amount of training data, and a high computational power. 
 
% Consequently, we propose to only learn generative model to build new instances for specific object classes, i.e., the ones with low segmentation accuracy. Let $m\in\mathbb{L}^{w \times h}$ be a semantic segmentation mask, where $w$ and $h$ represent its width and height, respectively. Our goal is to learn a mapping function that converts $m$ into a photo-realistic image. 


\subsection{cGAN Architecture}
\label{sec:cgan}

The first step of our approach concerns the generation of photo-realistic images of specific objects classes populating an agricultural scenes. We employ here the SPatially-Adaptive DEnormalization (SPADE) architecture~\cite{spade}, which is a type of conditional GAN (cGAN). Differently from other common cGANs, this type of network performs a Semantic Image Synthesis by converting a semantic segmentation mask into a photo-realistic image. In other words, its input/output behavior is the opposite of an image segmentation network. 

In the SPADE architecture, the image encoder encodes a real image into a latent representation for generating a mean and a variance vector. This allows to change the style (color, texture, etc.) of the image. The generator uses the segmentation map in each SPADE ResNet block. The discriminator takes a concatenation of the segmentation map with the original (or generated) image and it classifies it as real or fake.

The SPADE generator is built based on the pix2pixHD framework~\cite{wang2018high}. It starts with random noise in the input and uses the semantic map at every SPADE ResBlk upsampling layer. Also, using SPADE, it is possible:
\begin{itemize}
    \item to separate between semantic and style control;
    \item to change the final content, by modifying the semantic map;
    \item to change the style of the image, by modifying the random vector.
\end{itemize}

Also the discriminator architecture follows pix2pixHD and it uses a multi-scale design with instance normalization, with the difference that spectral normalization is applied to all the convolutional layers of the discriminator. In particular, it is based on Patch-GAN~\cite{isola2017image} and it takes as input the concatenation of the segmentation map with the image. The encoder is composed of six convolutional layers with stride 2 followed by two linear layers. It is responsible for producing the mean ($\mu$) and covariance ($\sigma^2$). 

Compared to its original version, we have made two major changes to the SPADE architecture. The first change is in the SPADE image synthesis modalities. The original version, indeed, takes as input RGB images and generates RGB images as well. In our case, to exploit the NIR channel, we enabled the network to work with 4 channel images, and thus to generate multi-spectral images. 
The second modification has been made in order to increase the size of the generated samples. The original version generates images with a resolution of 256$\times$256, which may not be enough to generate all the possible object classes. Differently, we generate images with a resolution of 512$\times$512.


\subsection{cGAN Evaluation Metrics}
\label{sec:gan_train_ev}

Evaluating GANs is a very challenging task and several aspects need to be taken into consideration when defining metrics that can produce meaningful scores. These metrics should be capable to distinguish between generated and real samples, to detect overfitting, and to identify mode dropping and mode collapsing. Our goal is to check whether the learned generative model well generalizes with respect to the problem of photo-realistic crop generation.

For most of the GANs presented in the literature, network inspection is qualitative only, based on a manual inspection to check the fidelity of the generated sample. This kind of evaluation is still considered the best approach, but it is time-consuming, subjective, and often it can also be misleading.

In this paper, we employ an empirical evaluation. The basic idea is to use samples generated by the network and samples collected from the real dataset to extract features from both of them, and then to calculate performance using specific metrics. In particular, we employ six metrics: Inception Score, Mode Score, Kernel MMD, Wasserstein distance, Fréchet Inception Distande (FID) and 1-nearest neighbor (1-NN). All the used metrics are described  in~\cite{Xu2018}. For space constraints, we describe here only the inception score, being the most popular metric for evaluating GANs.

\subsubsection{Inception.}
Inception is a metric capable of measuring not only the quality but also the diversity of generated images using an external model, the Google Inception network \cite{inception}, trained on the ImageNet dataset \cite{imagenet}.
The Inception Score can be calculated using the following formula
\begin{equation}
    \textrm{IS}(p_g)=e^{\mathbb{E}_{x \sim p_g}[KL(p_\mathcal{M}(y\mid\mathrm{x}) \parallel p_\mathcal{M}(y))]}
    \label{eq:inception}
\end{equation}

By considering a pretrained model $\mathcal{M}$, $p_\mathcal{M}(y\mid\mathrm{x})$ refers to the label distribution of $\mathrm{x}$ predicted by $\mathcal{M}$, and $p_\mathcal{M}(y)=\int_{\mathrm{x}}p_\mathcal{M}(y\mid\mathrm{x})dp_g$, which gives the marginal of $p_\mathcal{M}(y\mid\mathrm{x})$ over the probability measure $p_g$. The expectation and the integral in $p_\mathcal{M}(y\mid\mathrm{x})$ can be approximated with independent and identically distributed samples from $p_g$.

\subsection{Agricultural Scene Composition}
\label{sec:scene_gen}

The final step in our approach concerns using the crop and weeds RGB/NIR images described in Section~\ref{sec:cgan} to create a realistic agricultural scene. To do so, we follow the pipeline reported in Fig.~\ref{fig:segmentation_dataset}.

\begin{figure}[t]
 \centering
 \includegraphics[width=\linewidth]{images/synthetic_image_generation_1.png}
 \caption{Dataset creation for segmentation training. First the crop and weed masks are taken from the full mask, then new RGB and NIR crops and weed are generated from these masks and past back to the original image.}
 \label{fig:segmentation_dataset}
\end{figure}

First, we get the weed and crop masks from the full mask image. The mask is then resized to the SPADE network input size, which is 512$\times$512 pixels for crop and 128$\times$128 for weed given that weed tends to appear in smaller size than crop. The SPADE network then generates a random, photo-realistic, crop/weeds instance by using the shape of the input mask and a random noise signal. The generated image is then replaced into the source image. Fig.~\ref{fig:detail} shows an example of the obtained synthetic image. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/detail_reduced.png}
    \caption{An example of original image and the synthetic one obtained by inserting in the original image a plant sample generated using our cGAN.}
    \label{fig:detail}
\end{figure}




% \subsection{RGB Crop Image Generation}
% \label{sec:rgb_crop_gen}

% Consequently, we propose to only learn generative model to build new instances for specific object classes, i.e., the ones with low segmentation accuracy. Let $m\in\mathbb{L}^{w \times h}$ be a semantic segmentation mask, where $w$ and $h$ represent its width and height, respectively. Our goal is to learn a mapping function that converts $m$ into a photo-realistic image. 

% \subsection{NIR Image Generation}
% The original (SPADE) architecture~\cite{spade} used as input three layer RBG images and generates a three layer RGB image in the output, but in our case it was necessary to modify the network in a way that it works with a four layer image, three layers for the RGB (red, green and blue) and one layer for the NIR image. We concatenate rgb image with nir channel to get finally the four channels input. When evaluating the metrics it is also necessary to separate the output to have again two images, so the metrics are evaluated separately, even though being generated together by the same network.
% Before the concatenation process between rgb and NIR it was necessary to process the dataset in order to organize the images, to get perfect match between NIR pixels and RGB pixels. The RGB and NIR images are taken from the same camera, but because of small distortions, they first need to be undistorted using the camera matrices, provided by the dataset. It was noticed that even after undistorting the images they were one or two pixels off when superposing both, this displacement is not relevant for most applications, but in this case it was necessary to have a perfect match, because of this, it was decided to also apply a perspective transformation on NIR and NIR mask to get perfect match between RGB and NIR images.
% \begin{figure*}[t]
%  \centering
%  \includegraphics[width=0.92\linewidth]{images/NIR.png}
%  \caption{Image channel decomposition.}
%   \label{fig:channel_decomposition}
% \end{figure*}



% \subsection{GAN Training Evaluation}
% \label{sec:gan_train_ev}

% 

% \subsection{Scene Generation}
% \label{sec:scene_gen} 

% The final step in our approach is to use the crop RGB images described in Section~\ref{sec:rgb_crop_gen} to create a realistic agricultural scene. To do so, we follow the pipeline reported in Fig.~\ref{fig:segmentation_dataset}.
% First, we get the crop masks from the full mask image. The mask is then resized to the SPADE network input size, which is 256$\times$256 pixels. The SPADE network then generates a random, photo-realistic, crop instance by using the shape of the input mask and a random noise signal. The generated image is then up-sampled again to its original size and replaced into the source image.
% Despite the simplicity of the proposed approach, the up-sampling procedure may let the synthetic image to loose some details.
% Fig.~\ref{fig:detail} shows an example of the obtained synthetic image. 

% %The creation of a model to generate images of the proper size will be the subject of future investigations.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{images/detail.png}
%     \caption{Difference between the original image and the synthetic one obtained by inserting in the original image a plant sample generated using the GAN.}
%     \label{fig:detail}
% \end{figure}

==> olds/preliminaries.tex <==
\subsection{Generative Adversarial Networks}

Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} can estimate generative models through an adversarial training, which simultaneously train two networks:
\begin{enumerate}
    \item A generative model $G$, whose objective is to capture a data distribution.
    \item A discriminative model $D$ that outputs a single scalar, and whose objective is to estimate the probability that a sample is actually a real data and not synthetically generated by $ G $. 
\end{enumerate} 

Given any data distribution $p_{data}(x)$ and a prior input noise distribution $p_z(z)$ (which is typically uniform or Gaussian), the mapping to the data space is represented by $G(z)$, where $G$ is the generative model with its distribution $p_g$. Let us also define the discriminator $D$, as a function that outputs a single scalar. $D(x)$ represents the probability that $x$ comes from the real data space rather than $p_g$.

The training process is carried out by maximizing the probability of $D$ to assign a correct label to the generated and to the real samples, while $G$ is trained to learn the distribution $p_g$ over the data space $x$ so that $D$ can hardly assign them the correct label. $G$ and $D$ are trained in an unsupervised manner by a two-player min-max game that is given by:
\begin{equation}
    \min_{G} \max_{D} V(D,G) = \mathbb{E}_{x \sim p_{data}(x)}[logD(x)] + \mathbb{E}_{z \sim p_z(z)}[log(1-D(G(z))].
\end{equation}
where $\mathbb{E}$ and $log$ are the expectation and logarithmic operators, respectively. $D$ and $G$ are trained simultaneously until they cannot both improve because $p_g = p_{data}$, and the discriminator is unable to differentiate between the two distributions, i.e., $D(x) = 1/2$.  

\subsection{Conditional Generative Adversarial Networks}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/cGAN_scheme.png}
    \caption{ The cGAN generator learns a nonlinear function $G$ that maps an input mask (e.g., the shape of a plant) to a photo-realistic, in this work 4 channels, image. The cGAN discriminator learns a function $D$ that discerns real from synthesized images produced by $G$.}
    \label{fig:cgan_scheme}
\end{figure}

Conditional GANs (cGANs) \cite{Mirza2014cGANs} extend the GAN concept by conditioning both $D$ and $G$ through extra data $y$. It is worth noticing that $y$ can represent any kind of auxiliary information (in \cite{valerio2017arigan}, for instance, $y$ represents the number of leaves of the synthesised plant)
and it is fed into both the discriminator $D$ and generator $G$ as an additional input layer. With this new settings, $G$ attempts to synthesize realistic images $x$ from the $y$ domain, while $D$ receives samples from both $x$ and $y$ domains and attempts to discern between real-real and synthesised-real image pairs.
%samples from both domains (x and y) and attempts to discern between real-real and synthesized-real image pairs.
The cGAN scheme is shown in Fig. \ref{fig:cgan_scheme}. The loss function of cGANs can be expressed as
\begin{equation}
    \min_{G} \max_{D} V(D,G) = \mathbb{E}_{x \sim p_{data}(x)}[logD(x,y)] + \mathbb{E}_{z \sim p_z(z)}[log(1-D(G(z,y))]
\end{equation}

==> olds/relatedwork.tex <==
A robust crop/weed classification module is an essential component for autonomous farming robots as it enables the platform to properly perceive the environment and to carry out an efficient weed control policy. The problem has been extensively investigated over the years and it can be roughly split in two main categories:
\begin{enumerate}
    \item Classifiers based on hand-crafted features. %e.g.,\mbox{\cite{haug2014plant,lottesJFR2016,lottes2017icra}}
    \item Approaches using machine learning.
    %e.g., \mbox{\cite{dicicco2017,potena2016,mccool2017mixtures,mortensen2016semantic,milioto2019icra}}
\end{enumerate}    

Methods in the first group usually present limited generalization capabilities, dependent by the choice of the features to process.
The approaches in the second category have better generalization capabilities at the cost of annotating large datasets of images, which is a tedious and time-consuming process. In this section, we focus on crop/weed approaches belonging to the two above mentioned categories and we provide a discussion about methods that address the dataset annotation issue.

\subsection{Classifiers Based on Hand-crafted Features}
One of the the main goal of this class of methods is the choice of a suitable set of features that have good discrimination properties between the target plant classes.
Haug \textit{et al.}~\cite{haug2014plant} propose a plant classification method that is capable of distinguishing carrot and weeds by using RGB and near infra-red (NIR) images. The reported accuracy is around $93.8\%$. In \cite{lottesJFR2016}, the authors propose a sugar beets and weeds classification system based on a multi-spectral camera mounted on the robot. The method performs in sequence, a vegetation detection, an object-based features extraction, a random forest classification and a smoothing trough a Markov random field. Experiments have been carried out in different sugar beets field reporting good classification performance. The same method has been extended in \cite{lottes2017icra}, where the crop/weed classification data are acquired using a camera mounted on a light-weight UAV. The system has been tested in two farms in Germany and Switzerland, showing good generalization properties and the ability to classify individual plants.
Despite the promising results, the methods based on hand-crafted features are strictly dependent on the choice of features, which limits their generalization capabilities.

\subsection{Approaches Using Machine Learning}
Machine learning methods, and more specifically Convolutional Neural Networks (CNN), offer the potential to overcome the inflexibility of handcrafted vision pipelines, by allowing to develop effective end-to-end classification methods. In this regards, CNN are usually applied in pixel-wise fashion, operating on image patches provided by a sliding window approach. Following this idea, Potena \textit{et al.} \cite{potena2016} proposed a crop/weed classification architecture composed of a cascade of CNNs. The first CNN detects the vegetation, which is successively used as the input for a second, deeper, CNN that classifies vegetation pixels into crop or weeds.
McCool \textit{et al.}~\cite{mccool2017mixtures} propose a three stage approach. They start from a pre-trained model with state-of-the-art performance, but a high computational cost. Then, a model compression is performed, retrieving a faster CNN. Finally, they combine several lightweight models into a mixture model to enhance the performance. They report an accuracy around $93.9\%$. 

Differently from CNNs, Fully Convolutional Networks (FCN)~\cite{LongFCN2015} take as input images of arbitrary sizes and produce a correspondingly-sized segmented output without relying on local patches.
Among the many FCNs proposed in the literature, the most commonly adopted in crop/weed segmentation is SegNet \cite{Segnet}. In Di Cicco \textit{at al.}~\cite{dicicco2017}, the authors trained SegNet with real and synthetic images reporting a good segmentation performance. In \cite{weednet}, the authors used SegNet for dense semantic weed classification with multispectral images collected by a Micro Aerial Vehicle (MAV). A similar encoder-decoder architecture has been exploited in Milioto \textit{et al.}~\cite{miliotoicra2018} where the authors augmented the RGB input image with task-relevant background knowledge to speed up the training and to better generalize to new crop fields. We exploited a similar idea in our previous work~\cite{FawakherjiYBPN19}, where we propose a pipeline with multiple data channels to support the input of the CNN by using more vegetation indices. These additional information aid the CNN to achieve a good generalization to different crop types.

Lottes \textit{et al.}~\cite{lottes2018icra} propose a crop/weed classification system that, in addition to a fully convolutional network with an encoder-decoder structure, also exploits the crop arrangement information that is observable from the image sequences. This increases the segmentation performance and the generalization capabilities of the net to previously unseen fields under varying environmental conditions.
Mortensen \textit{et al.}~\cite{mortensen2016semantic} use a CNN to estimate the in-field biomass and crop composition. Their method is a modified version of the well-known VGG-16 deep neural network. The reported accuracy is $79\%$ with 7 classes of objects. Sa \textit{et al.}~\cite{sa2018weedmap} propose segmentation algorithm working on aerial images. The method exploits multi-spectral imagery and a CNN, reporting an error margin $\leq2\%$. 

\subsection{Labelling Effort Reduction}
The major drawback of CNNs and FCNs
architectures is that the level of expressiveness is limited by the size of the training dataset. In the context of precision farming, collecting large annotated datasets involves a significant effort. Datasets should be acquired across different growth stages and weather conditions. Moreover, the pixel-wise annotation process is tedious and extremely time consuming. As a matter of fact, the size of pixel-wise annotated datasets is usually relatively small \cite{xie2016}.

To cope with the above discussed problem, several solutions have been proposed in the literature. In~\cite{potena2016}, the authors propose a novel dataset summarization technique. The main idea is to summarize an original, unlabelled, dataset by taking only the most informative images. The summarized dataset will thus lead to a reduced labelling effort while keeping a sufficient segmentation performance. In Di Cicco \textit{et al.}~\cite{dicicco2017}, the authors propose to use a state-of-the-art graphic engine to generate synthetic and realistic farming scenes. The generated scene, together with their ground truth are used to train the final CNN or to supplement an existing real dataset.

Milioto \textit{et al.}~\cite{miliotoicra2018} propose a CNN that requires little data to adapt to the new unseen environment. The reported results show a segmentation accuracy around $96\%$ and a fast re-adaptation to new, unseen, environments. In \cite{weednet}, the authors dealt with the labelling effort by exploiting different fields with varying herbicide levels resulting in field patches containing only either crop or weed. This enables to exploit a simple vegetation index as a feature for automatic ground truth generation.
Although the methods described so far can successfully mitigate the annotation effort issue, they may not yet achieve the segmentation performance of a fully trained FCN.

More recent approaches make use of GANs. Giuffrida \textit{et al.}~\cite{valerio2017arigan} exploit a conditional GAN to generate $128\times128$ synthetic \textit{Arabidopsis} plants, with the possibility to decide the desired number of leaves of the final plant. Their method has been tested by using a leaf counting algorithm showing how the addition of synthetic data helps to avoid overfitting and to improve the accuracy. In \cite{MADSEN2019147}, the authors leverage a GAN to generate artificial image samples of plant seedlings to mitigate for the lack of training data. The proposed method is capable to generate 9 distinct plant species while increasing the overall recognition accuracy.
Unlike the last method, in this work we propose to generate \emph{multi-spectral} views of agricultural scenes by synthesizing only the objects that are relevant for semantic segmentation purposes.

==> olds/results.tex <==
A quantitative evaluation has been carried out to show that by augmenting the training datasets of state-of-the-art segmentation networks with synthetic photo-realistic images generated with our model allows to: i) Improve the networks generalization capabilities, and; ii) Increase the performance in crop/weed segmentation.
Moreover, the annotation effort is limited, since the cGAN generates both the images and the masks.    
\begin{figure}[!t]
    \centering
    \includegraphics[width=.7\columnwidth]{images/dataset.png}
    \caption{First row: examples of RGB image from Stuttgart (left) and Bonn (right) datasets. Second row: examples of data used to train SPADE for weed. From left to right, RGB, NIR, and mask samples, respectively. Third row: examples of data used to train SPADE for crop. From left to right, RGB, NIR, and mask samples, respectively.}
    \label{fig:results}
\end{figure}


\subsection{Training and Testing Data}

To test our approach, we used two open-source sugar beet datasets: Bonn dataset and Stuttgart dataset~\cite{chebrolu2017ijrr}. Both the datasets have been collected by a BOSCH Bonirob farm robot (see Fig.~\ref{fig:teaser_img}, top row) moving on a sugar beet field across different weeks. The datasets are composed of images taken by a 1296$\times$966 pixels 4-channels (RGB-NIR) JAI AD-13 camera, mounted on the robot and facing downward. 

We created four different datasets:
\begin{enumerate}
\item \textit{Original}, which is a reduced version of the Bonn dataset. We took a total of 1600 images from the  Bonn dataset, randomly chosen among different days of acquisition in order to contain different growth-stages of the target crop. Then, we split it into a training set (1000 images), a validation set (300 images), and a test set (300 images). 
\item \textit{Synthetic Crop}, composed of 1000 images with synthetic crop generated by using our architecture.
\item \textit{Synthetic Weed}, composed of 1000 images with synthetic weeds generated by using our architecture.
\item \textit{Mixed}, containing 2000 images and composed by the union of 1000 images from the Original dataset and 1000 images with synthetic crop and weeds.
\end{enumerate}

For testing, we used 300 real images from Stuttgart dataset and 300 real images (not used for training) from Bonn dataset. It is worth noting that we used the Stuttgart dataset to show the improvement in the generalization capability of the segmentation net after augmenting the training dataset with our approach.

We point out that, in the synthetic datasets, we replaced with synthetically generated plants only plants whose stem is totally framed into the image. For plants that are mostly out of the frame, the original one is kept. We experimentally verified that it is necessary to have the stem of the plant roughly in the center the mask to obtain an effective synthetic image generation.


\subsection{Evaluation of the Semantic Segmentation}

We used the four datasets described above to train four state-of-the-art semantic segmentation networks, namely Unet \cite{Unet}, Unet-resnet (Unet with Resnet50 back-end), Bonnet \cite{milioto2019icra}, and Segnet \cite{Segnet}.
To evaluate the semantic segmentation output, we used the following metrics: Per-class Intersection over Union, Average Intersection over Union (denoted as \textit{mIoU}), Per-class Recall, and Per-class Precision. 
An example of segmentation results is shown in Fig.~\ref{fig:pred_ex}.

\begin{figure}
    \centering
    \includegraphics[width=.95\columnwidth]{images/isa_output.png}
    \caption{Examples of a segmented image obtained by using four different segmentation networks trained with three different datasets. The first row of the image shows the input RGB, NIR images and its corresponding ground truth. The remaining rows show the segmentation results generated by the different networks on the $Original$, $Synthetic$, and $Mixed$ training datasets.}
    \label{fig:pred_ex}
\end{figure}

\begin{table}[!h]
\centering
\caption{ Pixel-wise  segmentation performance, RGB input, trained on four different datasets, tested on part of Bonn dataset.}
\begin{tabular}{c c c c c c c c c c c c}
 \hline
      Dataset & FCN    & MIoU   & \multicolumn{3}{c}{IOU} & \multicolumn{3}{c}{Recall} &\multicolumn{3}{c}{Precision} \\  \cline{4-6} \cline{8-9} \cline{11-12}
            &     &      & Soil   &  Crop  &  Weed & &  Crop  &  Weed & &  Crop  &  Weed\\  \hline

\multirow{4}{*}{\textit{synthetic weed}}
     &\textit{Bonnet}      & 0.65 & 0.99 & 0.64 & 0.31  & & 0.71 & 0.53 & & 0.64 & 0.38 \\   %\cline{2-12}
     &\textit{Unet-resnet} & 0.64 & 0.99 & 0.73 & 0.18  & & 0.73 & 0.20 &  & 0.86 & 0.30 \\ 
     %\cline{2-12}
     & \textit{Unet}       & 0.63 & 0.99 & 0.71 & 0.19 &  & 0.74 & 0.19 &  & 0.93 & 0.35 \\  %\cline{2-12}
     & \textit{Segnet}     & 0.61 & 0.99 & 0.60 & 0.14 &  & 0.72 & 0.18 &  & 0.86 & 0.47 \\  \hline
\multirow{4}{*}{\textit{synthetic crop}}&\textit{Bonnet } &0.67&  0.99  & 0.73  & 0.30 &    & 0.93  & 0.49   &  & 0.73   & 0.45 \\ %\cline{2-12}
& \textit{Unet-resnet} &   0.69 & 0.99  & 0.79 & 0.29 &   & 0.81  & 0.33   &   & 0.96   & 0.18 \\  %\cline{2-12}
&\textit{Unet }  & 0.65 & 0.99  & 0.76  & 0.20 &   & 0.81  & 0.37   &  & 0.98   & 0.37 \\  
%\cline{2-12}
&\textit{Segnet }   & 0.64& 0.99  & 0.74  & 0.17 &   & 0.80  & 0.21   &  & 0.91   & 0.48  \\  
\hline

\multirow{4}{*}{\textit{Original}}
& \textit{Bonnet}    & 0.70 & 0.99 & 0.75 & 0.35 &  & 0.84 & 0.54 & & 0.82 & 0.49 \\ %\cline{2-12}
&\textit{Unet-resnet}& 0.67 & 0.99 & 0.81 & 0.23 &  & 0.95 & 0.25 &  & 0.95 & 0.63 \\  %\cline{2-12}
& \textit{Unet}      & 0.68 & 0.99 & 0.82 & 0.22 & & 0.84 & 0.26 &  & 0.95 & 0.64 \\  %\cline{2-12}
& \textit{Segnet}    & 0.66 & 0.99 & 0.78 & 0.20 & & 0.81 & 0.37 & & 0.97 & 0.37  \\  \hline

\multirow{4}{*}{\textit{Mixed}}
&\textit{Bonnet} &  \textbf{0.76} &  0.99  &  \textbf{0.92}  & \textbf{0.38} &    & \textbf{0.96}  & \textbf{0.58}   & & 0.95   & 0.56 \\ %\cline{2-12}
&\textit{Unet-resnet} &  0.72 & 0.99  & 0.85  & 0.32 &   & 0.87  & 0.45   & & 0.97   & 0.48  \\  %\cline{2-12}
&\textit{Unet} & 0.71& 0.99  &0.87  & 0.27 &   & 0.89  & 0.28   & & \textbf{0.97}   & \textbf{0.72} \\  %\cline{2-12}
&\textit{Segnet}  &0.70 & 0.99  & 0.85  & 0.26 &   & 0.88  & 0.40   & & 0.96   & 0.49 \\  \hline

\end{tabular}
\label{tab:bonnet_segmentation_results}
\end{table}


\begin{comment}
 \begin{table}[!h]
\caption{Pixel-wise segmentation performance obtained by training on two different inputs (RGB) and (RGB + NIR) and tested on two different datasets.}
\begin{tabular}{ c  c  c  c   c| c  c  c| c  c  c| c  c  c}
 \hline
 Train set & Test set & \multicolumn{3}{c }{Bonnet} & \multicolumn{3}{c}{Unet-resnet}& \multicolumn{3}{c}{Unet}&\multicolumn{3}{c}{Segnet} \\ 

     &      &     & \multicolumn{2}{c  }{IOU}&   & \multicolumn{2}{c  }{IOU}&    & \multicolumn{2}{c  }{IOU}&    & \multicolumn{2}{c}{IOU}   \\ 
           &     &  MIoU        &  Crop  &  Weed&  MIoU     &  Crop  &  Weed & MIoU     &  Crop  &  Weed & MIoU     &  Crop  &  Weed  \\   \hline


\multirow{2}{*}{\textit{Original }} 
        & \textit{Bonn }   &0.77 &   0.85 & 0.45      &0.31 & 0.85 & 0.35   &0.69  & 0.84 & 0.24 &0.69 & 0.84 & 0.25 \\ %\cline{2-18}

       & \textit{Stuttgart } &0.49 &  0.32 & 0.12     &0.47 & 0.30 & 0.15  &0.45  & 0.34 & 0.13 &0.41   & 0.27 & 0.11  \\  \hline
        
\multirow{2}{*}{\textit{Mixed} }
        & \textit{Bonn }  &0.83 &  0.94 & 0.55       &0.77  & 0.92 & 0.40   &0.74  & 0.85 & 0.37 &0.73   & 0.88  & 0.30    \\   %\cline{2-18Pixel-wise segmentation performance , trained on two different inputs (RGB) and (RGB + NIR), tested on two different dataset.}

        & \textit{Stuttgart }   &0.57 &   0.46 & 0.28   &0.54  & 0.52 & 0.16   &0.53  & 0.50 & 0.19 &0.51   & 0.47  & 0.14    \\  \hline
 \end{tabular}
 \label{tab:Multi-channel-Stuttgart_segmentation_results}
 \end{table}

\end{comment}







 
\begin{table}[!h]
\caption{Pixel-wise segmentation performance , trained on two different inputs (RGB) and (RGB + NIR), tested on two different dataset.}
\begin{center}
\begin{tabular}{ c  c  c  c   c| c  c  c| c  c  c }
 \hline
 Train set & Test set 
                     &\multicolumn{3}{c }{Bonnet}
                     &\multicolumn{3}{c}{Unet-resnet}
                     &\multicolumn{3}{c}{Unet}
                      \\ 
            &        &     
                     & \multicolumn{2}{c  }{IOU}
            &        & \multicolumn{2}{c  }{IOU}
            &        & \multicolumn{2}{c  }{IOU}    \\ \cline{4-5}\cline{7-8}\cline{10-11} 
            &        & MIoU & Crop & Weed   & MIoU & Crop & Weed    & MIoU & Crop & Weed \\   \hline


   \textit{Original}  
        & \textit{Stuttgart  } 
               & 0.30 & 0.13 & 0.1 
               & 0.31 & 0.11 & 0.12 
               & 0.33 & 0.14 & 0.08 
                  \\
       \scriptsize \textit{(RGB)}      
         & \textit{Bonn}  
               & 0.70 & 0.75 & 0.35
               & 0.67 & 0.81 & 0.23
               & 0.68 & 0.82 & 0.22      \\ \hline
      \textit{Mixed } 
         & \textit{ Stuttgart  }
               & 0.38 & 0.26 & 0.18 
               & 0.35 & 0.2  & 0.13  
               & 0.37 & 0.21 & 0.15
                \\
     \scriptsize \textit{(RGB)}
        & \textit{Bonn}
               & 0.76 & 0.92 & 0.38
               & 0.72 & 0.85 & 0.32
               & 0.71 & 0.87 & 0.27
                 \\ \hline
       \textit{Original} 
            & \textit{Stuttgart } 
               & 0.49 & 0.32 & 0.12 
               & 0.47 & 0.30 & 0.15
               & 0.45 & 0.34 & 0.13 
                 \\
        \scriptsize \textit{ (RGB+NIR) } 
              & \textit{Bonn} 
               & 0.77 & 0.85 & 0.45
               & 0.31 & 0.85 & 0.35 
               & 0.69 & 0.84 & 0.24
                \\ \hline
         
                  
  \textit{Mixed} 
               & \textit{ Stuttgart } 
               &\textbf{ 0.57} & 0.46 & \textbf{0.28}
               & 0.54 & \textbf{0.52} & 0.16
               & 0.53 & 0.50 & 0.19 
                  \\  
 \scriptsize \textit{(RGB+NIR) }
            & \textit{Bonn } 
               &\textbf{0.83}  & \textbf{0.94} &\textbf{0.55}  
               & 0.77 & 0.92 & 0.40
               & 0.74 & 0.85 & 0.37 
                  \\  \hline

       
\end{tabular}
\end{center}
\label{tab:Multi_channel_segmentation_results}
\end{table}

\begin{table}[!h]
\centering
\caption{ Pixel-wise segmentation performance for sunflower dataset, trained on two different inputs (RGB) and (RGB + NIR).}
\begin{tabular}{c c c c c c c c c c c c}
 \hline
      Dataset & FCN    & MIoU   & \multicolumn{3}{c}{IOU} & \multicolumn{3}{c}{Recall} &\multicolumn{3}{c}{Precision} \\  \cline{4-6} \cline{8-9} \cline{11-12}
            &     &      & Soil   &  Crop  &  Weed & &  Crop  &  Weed & &  Crop  &  Weed\\  \hline


\multirow{2}{*}{\textit{synthetic crop}}
  &\textit{Bonnet } &0.76&  0.99  & 0.84  & 0.46 &    & 0.94  & 0.61   &  & 0.88   & 0.67 \\ %\cline{2-12}
   &\textit{Unet } &0.51&  0.98  & 0.038  & 0.51 &    & 0.039  & 0.51   &  & 0.57   & 0.98 \\ %\cline{2-12}
 \textit{(RGB)}   &\textit{Unet-resnet } &0.53&  0.98  & 0.05  & 0.59 &    & 0.05  & 0.63   &  & 0.32   & 0.89 \\ %\cline{2-12}
  
%\textit{(RGB)}&\textit{ } & &   &   &  &    &  &  &  &  & \\ %\cline{2-12}
\hline
\multirow{2}{*}{ \textit{synthetic crop }   }&\textit{Bonnet} &   0.83 & 0.99  & 0.84 & 0.66 &   & 0.97  & 0.81   &   & 0.85   & 0.78 \\  %\cline{2-12}

 &\textit{Unet } &0.701&  0.99  & 0.69  & 0.41 &    & 0.81  & 0.45   &  & 0.83   & 0.87 \\ %\cline{2-12}
 \textit{(RGB+NIR)}   &\textit{Unet-resnet } &0.704&  0.99  & 0.65  & 0.47 &    & 0.73  & 0.52   &  & 0.86   & 0.82 \\ %\cline{2-12}
\hline

\multirow{2}{*}{\textit{Original}}
& \textit{Bonnet}    & 0.70 & 0.99 & 0.82 & 0.30 &  & 0.94 & 0.61 & & 0.86 & 0.23 \\ %\cline{2-12}
 &\textit{Unet } &0.39&  0.97  & 0.15  & 0.031 &    & 0.17  & 0.04   &  & 0.72   & 0.10 \\ %\cline{2-12}
 \textit{(RGB)}   &\textit{Unet-resnet } &0.43&  0.98  & 0.28  & 0.04 &    & 0.34  & 0.06   &  & 0.65   & 0.08 \\ %\cline{2-12}
\hline
\multirow{2}{*}{ \textit{Original} }
& \textit{Bonnet}    & 0.80 & 0.99 & 0.78 & 0.62 &  & 0.87 & 0.82 &  & 0.88 & 0.71 \\ %\cline{2-12}
&\textit{Unet } &0.64&  0.99  & 0.54  & 0.38 &    & 0.70  & 0.42   &  & 0.83   & 0.40 \\ %\cline{2-12}
 \textit{(RGB+NIR)}   &\textit{Unet-resnet } &0.66&  0.99  & 0.60  & 0.43 &    & 0.75  & 0.49   &  & 0.88   & 0.90 \\ %\cline{2-12}
\hline
 
 

\multirow{2}{*}{\textit{Mixed} }
&\textit{Bonnet} & 0.78 &  0.99  & 0.87  & 0.48 &    & 0.95  & 0.59 & & 0.91   & 0.73 \\ %\cline{2-12}
 &\textit{Unet} &0.59 &  0.98  & 0.64  & 0.12 &    & 0.71  & 0.12 & & 0.88   & 0.98 \\ %\cline{2-12}
\textit{(RGB)}&\textit{Unet-resnet} &0.60 &  0.98  & 0.67  & 0.15 &    & 0.74  & 0.14 & & 0.90   & 0.97 \\
\hline


\textit{Mixed}
&\textit{Bonnet} &  0.86 & 0.99  & 0.88  & 0.69 &   & 0.97  & 0.85   & & 0.90   & 0.79  \\ %\cline{2-12}
&\textit{Unet} &  0.69 & 0.99  & 0.68  & 0.40 &   & 0.80  & 0.43   & & 0.83   & 0.87  \\ %\cline{2-12}
\textit{(RGB+NIR)} &\textit{Unet-resnet} &  0.72 & 0.99  & 0.70  & 0.48 &   & 0.77  & 0.51   & & 0.88   & 0.87  \\
\hline

\end{tabular}
\label{tab:sunflower_segmentation_results}
\end{table}




\begin{comment}
 \begin{figure*}
\centering
    \includegraphics[width=.85\columnwidth]{images/output_examples/rgb.png}
    \includegraphics[width=.85\columnwidth]{images/output_examples/groundTruth.png}\\\vspace{.25cm}
    \includegraphics[width=.6\columnwidth]{images/output_examples/bonnet_real.jpg}
    \includegraphics[width=.6\columnwidth]{images/output_examples/segnet_real.png}
    \includegraphics[width=.6\columnwidth]{images/output_examples/Unet_real.png}\\\vspace{.25cm}
    \includegraphics[width=.6\columnwidth]{images/output_examples/bonnet_synth.jpg}
    \includegraphics[width=.6\columnwidth]{images/output_examples/segnet_synth.png}
    \includegraphics[width=.6\columnwidth]{images/output_examples/Unet_synth.png}\\\vspace{.25cm}
    \includegraphics[width=.6\columnwidth]{images/output_examples/bonnet_synth_real.jpg}
    \includegraphics[width=.6\columnwidth]{images/output_examples/segnet_synth_real.png}
    \includegraphics[width=.6\columnwidth]{images/output_examples/Unet_synth_real.png}
    \caption{Examples of a segmented images obtained by using three different segmentation networks trained with three different datasets. The first row of the image shows the starting image and its corresponding ground truth. The second row shows the segmentation results obtained with Bonnet, Segnet, and Unet using the $Original$ dataset for training. The third and forth rows
    show the segmentation results obtained using the $Synthetic$ and $Mixed$ training datasets, respectively.}
    \label{fig:pred_ex}
\end{figure*}
\end{comment}




Table  \ref{tab:bonnet_segmentation_results} shows the quantitative results of   the semantic segmentation on real images held out from Bonn dataset. For all the architectures,  the results show that the IoU increases drastically by using the original dataset augmented with the synthetic ones compared to using only the original dataset. Moreover, using only the synthetic dataset also leads to a competitive performance when compared with using only the original one. In the case of the Unet-Resnet architecture, using only the synthetic dataset overcomes the performance obtained by using only the original one.

To show the improvements in generalization capability, we also used the Stuttgart dataset as test data. For all the tested architectures, the generalization capability improved when using the \textit{Mixed} dataset, i.e., when the dataset containing real images is augmented with synthetic data (see Table \ref{tab:Multi_channel_segmentation_results}).

The benefits of using an augmented dataset have also been demonstrated in the case of RGB plus NIR images. In this experiment, we used four channels images as input to train all the considered architectures on both \textit{Original} and \textit{Mixed} datasets.
Results are reported in the second part of Table \ref{tab:Multi_channel_segmentation_results}. Using the \textit{Mixed} RGB plus NIR dataset during the training process leads to a better generalization. In fact, the segmentation performance increases in all the considered setups. 
%The network that reports the highest performance increment is Bonnet, with an almost constant factor in its segmentation performance of $7\%$ and $19\%$ in the Bonn and Stuttgart datasets, respectively. 
This proves our claim that also the NIR channel generated using our approach improves the generalization capability of all the convolutional network architectures used in our experiments.

All the datasets generated using the approach described in this work are publicly available and can be downloaded from:\\
\url{https://bit.ly/3dSLEfZ}



